Bit Error Probability Instead of Secrecy Rate Criterion to Enhance Performance for Secure Wireless Communication Systems

In this paper, we propose a new practical power allocation technique based on bit error probability (BEP) for physical layer security systems. It is shown that the secrecy rate that is the most commonly used in physical layer security systems, cannot be a suitable criterion lonely. Large positive values are suitable for the secrecy rate in physical layer security, but it does not consider the performance of the legitimate and adversary users. In this paper, we consider and analyze BEP for physical layer security systems because based on it, the performance of the legitimate and adversary users are guaranteed and it is needed to use lower power. BEP is calculated for the legitimate and adversary users and it is shown that BEP can be better criterion for performance evaluation of the physical layer security systems. Based on BEP, the optimum transmit power is obtained and a new definition for outage probability is proposed and obtained theoretically. Also, the proposed approach is applied for adversary users with unknown mode and the cooperative adversary users. Simulation results show that the proposed method needs more than 5dB lower power for different scenarios.

==> BER <==
\relax 
\@writefile{toc}{\contentsline {section}{\numberline {I}Introduction}{1}}
\newlabel{Introduction}{{I}{1}}
\@writefile{toc}{\contentsline {section}{\numberline {II}The secrecy rate and study motivation}{2}}
\newlabel{motivation}{{II}{2}}
\newlabel{RS}{{1}{2}}
\@writefile{toc}{\contentsline {section}{\numberline {III}Proposed BEP based power allocation }{3}}
\newlabel{power allocation}{{III}{3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {III-A}}BPSK signaling}{3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {III-B}}QPSK signaling and the other type of modulations}{4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {III-C}}Multiple adversary users’ case}{5}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {III-D}}Adversary users with unknown mode}{5}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {III-E}}Cooperative adversary users}{6}}
\@writefile{toc}{\contentsline {section}{\numberline {IV}Improving outage probability by using multiple antennas transmitter and channel coding}{7}}
\newlabel{multiple antennas}{{IV}{7}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {IV-A}}Multiple antenna transmitter and sending artificial noise}{7}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {IV-B}} Channel coding}{7}}
\@writefile{lot}{\contentsline {table}{\numberline {I}{\ignorespaces Simulation parameters\relax }}{8}}
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{table}{{I}{8}}
\@writefile{toc}{\contentsline {section}{\numberline {V} Simulation results}{8}}
\newlabel{results}{{V}{8}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces The secrecy rate \textit  {vs}. Transmit power.\relax }}{8}}
\newlabel{1}{{1}{8}}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces BEP \textit  {vs}. Transmit power.\relax }}{8}}
\newlabel{2}{{2}{8}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces The optimum power value for different number of the adversary users.\relax }}{8}}
\newlabel{3}{{3}{8}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces The outage probability for different number of the adversary users.\relax }}{9}}
\newlabel{4}{{4}{9}}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces The optimum power value for cooperative adversary users and unknown mode.\relax }}{9}}
\newlabel{5}{{5}{9}}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces The outage probability for cooperative adversary users and unknown mode.\relax }}{9}}
\newlabel{6}{{6}{9}}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces Outage probability with channel coding.\relax }}{9}}
\newlabel{7}{{7}{9}}
\bibcite{1}{1}
\bibcite{2}{2}
\bibcite{3}{3}
\bibcite{4}{4}
\bibcite{5}{5}
\bibcite{6}{6}
\bibcite{7}{7}
\bibcite{8}{8}
\bibcite{9}{9}
\bibcite{10}{10}
\bibcite{11}{11}
\bibcite{12}{12}
\bibcite{13}{13}
\bibcite{14}{14}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces Outage probability with using beamforming and sending artificial noise.\relax }}{10}}
\newlabel{8}{{8}{10}}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces BEP of the legitimate and adversary users.\relax }}{10}}
\newlabel{9}{{9}{10}}
\@writefile{toc}{\contentsline {section}{\numberline {VI}Conclusion}{10}}
\newlabel{Conclusion}{{VI}{10}}
\@writefile{lof}{\contentsline {figure}{\numberline {10}{\ignorespaces BEP of the legitimate and adversary users by using beamforming and artificial noise.\relax }}{10}}
\newlabel{10}{{10}{10}}
\@writefile{toc}{\contentsline {section}{References}{10}}
\bibcite{15}{15}
\bibcite{16}{16}
\bibcite{17}{17}
\bibcite{18}{18}
\bibcite{19}{19}
\bibcite{20}{20}
\bibcite{21}{21}
\bibcite{22}{22}
\bibcite{23}{23}
\bibcite{24}{24}
\bibcite{25}{25}
\bibcite{26}{26}
\bibcite{27}{27}
\bibcite{28}{28}
\bibcite{29}{29}
\bibcite{30}{30}
\bibcite{31}{31}
\bibcite{32}{32}
\bibcite{R5}{33}

